Dynamic Programming for Symbolic Boolean Realizability and Synthesis

Inspired by recent progress in dynamic programming approaches for weighted model counting, we investigate a dynamic-programming approach in the context of boolean realizability and synthesis, which takes a conjunctive-normal-form boolean formula over input and output variables, and aims at synthesizing witness functions for the output variables in terms of the inputs. We show how graded project-join trees, obtained via tree decomposition, can be used to compute a BDD representing the realizability set for the input formulas in a bottom-up order. We then show how the intermediate BDDs generated during realizability checking phase can be applied to synthesizing the witness functions in a top-down manner. An experimental evaluation of a solver -- DPSynth -- based on these ideas demonstrates that our approach for Boolean realizabilty and synthesis has superior time and space performance over a heuristics-based approach using same symbolic representations. We discuss the advantage on scalability of the new approach, and also investigate our findings on the performance of the DP framework.

==> sections/other/notes.tex <==

\section{Fmcad notes: not formal section}

0. general BDDs: from binary decision tree, path to 1-terminal = a sat assignment, reduce subgraphs, reduce both edges

1. conjoin factor BDDs, and synthesize and eliminate variables that do not appear in later conjunts

2. given are $B, X, Y$, $Y_i$ takes those $y_i$'s with last occurrences in conjunct

3. k is the number of factored conjuncts

4. $P_i = (\exists {y_j1})(\exists {y_j2})... 1 \land B_1 \land ... B_i$, where $y_{j1}, y_{j2}, ...$ are all from $Y_1...Y_i$

5. clusters:  conjunction of partitioned conjuncts, first find witnesses inside each cluster of $f_i$'s?

6. rank of $f_i$: the highest index of y variable in its support

7. rank-based clustering: cluster factors by $C_1, ..., C_{\kappa}$ by ranks

8. reordering heuristics: Bouquet's method (rank low->high), Bucket elimination (rank high->low), Forward (select next factor: the one having most variables not in the rest of factors), Backward (select next factor: the one with fewest new variables than previous factors, to reduce size of conjoined BDD)

9. ordering heuristic selected: inverse MCS: in Gaifman graph (1 vertex per input/output variable, 1 edge between two vertices if both variables occur in the support of some same factor), inverse of the order that selects next variable that has the most same-support edges with previous variables

10. Fmcad 17: input $(\forall x)(\exists y)CNF$, see each clause as a factor, use CUDD's monolithic synthesis function $SolveEqn$ used for synth in algorithm

Notes:

1. initial empty conjunction = constant 1? Does it mean tautology and its BDD is just the 1-terminal? yes

2. no orders inside clusters, ordering/reordering heuristics are just for ordering the clusters after assigning factors to clusters

3. witnesses found in clusters (when the algorithm is applied to each cluster) are the same as witnesses for the overall CNF?

4. Do we use just one variable $p$ in BDDs to represent both $p$ after 1-edges and $\neg p$ after 0-edges (unlike two nodes $p$ and $\neg p$ like in ZDDs)?

\section{Procount notes: not formal section}
1. weighted projected model count W-weighted Y-projected $WPMC(\phi, W, Y)$ = weighted (over weights of truth assignments to X) sum of maximal value of Y (over all possible truth assignments on Y)?

2. literal weight function assigns to x and -x real values?

3. $\delta_G$ assigns to each vertex a set of edges, and $\epsilon_G$ assigns to each edge a set of vertices?

4. Projected MC: partition variables into X,Y\\weighted MC: has a weight function

5. Project-join tree:

1) children nodes of node $n$ in Tree $T$ with root $r$: $\mathcal{C}_{T,r}(n)$, leaves (degree 1) $\mathcal{L}(T)$

2) leaves = clauses ($\gamma: \mathcal{L}(T) \rightarrow \phi$), internal nodes = additive projections ($\pi$ assigns to each internal nodes a set of variables, and the two sets of variables labelled by two different internal nodes have no overlapping variables, and the internal nodes make a partition of variables

3) every leave of a clause containing variable x must be children/grandchildren node of the internal node labelling x

6. can compute W-valuation of a node $f_n^W$, if given Project-join tree and literal weight function over X; the W-valuation of leave nodes are just the clauses they represent, and the W-valuation of internal nodes = (the product of W-valuations of all its children nodes * the product of the weights of variables it labels) then do additive projection on all variables it labels

Finally the root's W-valuation is just the weighted model count.

Question: the literal-weight function domain includes both x's and y's?

7. size(n) = |Vars(n)|, width(T) = max of size(v) over V


8. Graded project-join tree:
1) internal nodes (including root) partitioned into $I_X, I_Y$, the x's nodes are never descendants of y's nodes ($I_X$ nodes closer to root than $I_Y$ nodes)

9. given graded project-join tree and weight function, can compute W-projected valuation for a node $g_n^W$. For leave nodes $g_n^W$ is the represented clause, and for internal nodes in $I_X$ it is similar to $f_n^W$, for internal Y nodes it is (product of $g_n^W$ of all its children nodes) then do existential projections (quantification) on all variables it labels

The final value of $g_{root}^W$ is weighted projected model counting.

10.free project-join tree -> reduce-> build ungraded project-join tree: 1) free variables are labelled at root: first ignore free variables, then add at root->not guarantee width to be smallest; first make project-join tree of $\phi  \cup$ virtual clause(of free variables) rotate without changing widths

2) partition clauses based on Y, make project-join trees, which is free on x's and all variables not labelled not also in children nodes. Then project all y's in Y, Then combine trees and project X's, 

Question: what are our free variables after projecting out all Y's?

\section{Questions:}
1. if X 
solved

Question: the empty set in $f_r^W(\emptyset)$ is there because the root node always labels the empty set?

Question: Vars(n) for internal nodes are those that appear in the same clauses with the variables it labels, but are not labelled by it?


==> sections/other/removedHeuristics.tex <==
 %\item Which variable ordering gives the best time performance for DPSynth?
    
    %\yi{to be determined}\item Are there some winning heuristics for ordering variables in conjunction and projection inside an internal node?
    
    %\item In the tree-based dynamic approach, how do low tree-width and high tree-width affect the performance in realizability checking, and are there patterns between time or space cost to tree-widths?
    
    %In our implementation we order the variables in the BDDs by multiple heuristics. This basic approach ordering them by MCS ordering, which utilizes the Gaifman graph. In short, the more variables a variable has co-occurrences with in some clauses, the higher the variable is ordered. Moreover, we select each clause as a cluster, i.e., a leave, as in line 9 of Algorithm.~\ref{alg: high valuation}, so that the realizability checking procedure directly ensures that whenever a \emph{pre-valuation} is equivalent to $\llbracket 0 \rrbracket$, it follows from the semantics of clauses that null realizability is obvious, and this trivial clustering heuristics is intuitively consistent with graded-tree approaches in a trivial perspective.

%The second variant of DPSynth approach applies heuristics from the graded-tree structure itself. We call it \emph{leave-to-root ordering}, in that we construct all BDD representations through out the solving procedure by ordering the variables exactly in the order they appear in labels of internal nodes, from the lowest level of internal nodes to the root. For variable in the same level of the tree that have equal distance to the root node, we break the ties by ordering them according to MCS ordering in the BDDs. This ordering from leave to root allows us to project out those variables that depend on less clauses more easily as they occur closer to the root in BDDs. 

%In order to investigate whether or not our intuitive speculation, which in short states that projections are faster when the projected variables are closer to the root node of BDDs, is correct, we also experimented on another ordering: the reverse of the above. We call it \emph{root-to-leave ordering}. The BDDs take variable orders from labels of higher level internal nodes and gradually to the lowest level internal nodes. Similarly, we order variables in the same level of labels in the graded project-join tree by MCS. In this case the higher a variable is labelled in the project-join graded-tree, the closer it is in BDDs.


%The orderings mentioned above are for variables in BDDs. We are also interested in the ordering to select BDDs to conjoin, as well as the ordering to pick variables in a label to project out. Hence experiments on \emph{conjoining heuristics} and \emph{projecting heuristics} are also included. For conjoining heuristics, we compare four different heuristics: increasing and decreasing indices, as well as small-size first and large-size first. In projecting heuristics comparison, we evaluate four variable heuristics: increasing and decreasing indices, and MCS and inverse-MCS orderings.

% Among permutation heuristics of variables, the MCS ordering, compared with the leave-to-root ordering in Figure.~\ref{figure: Leave-to-root vs. MCS Ordering Realiz Time }, shows strengths in time complexity. Although the total time taken by checking realizability is negligible, in most cases leave-to-root ordering exhausts more time than MCS by a relatively observable portion of the total time span.

% This also shows that MCS ordering, when applied appropriately, can function to improve the graded-tree based approaches in synthesis solving, besides its usage for model counting works~\cite{dudek2020dpmc, Procount}. Among tree-based dynamic solutions, leave-to-root and root-to-leave orderings interpret the the given specification to the most extent from \emph{tree} perspective, while MCS DPSynth shows the synthesis and model counting using tree-based approaches have similar preferences over variable orderings. \yi{the above paragraphs new}

==> sections/other/sketch.tex <==
\section{sketch - not formal section}
\subsection{Realizability}

Given: CNF $\phi, Vars(\phi), X, Y$

Can compute: tree decomposition of Gaifman graph of $\phi$, ungraded project-join tree, X-free project-join tree, Graded project-join tree, ordering heuristics, clustering heuristics

Do: 
\begin{enumerate}
    \item compute the graded project-join tree, each leave represents a clause
    \item compute BDD for every leave/clause
    \item initial B = 1-terminal
    \item in every iteration, conjunct B with the BDD for a leave/clause's BDD, following the tree, eliminate y's whenver an internal node's all children leaves are conjuncted
    \item get the final BDD representing realizable set
    \item if is 1-terminal, tautology, meaning full realizability
    \item if not 1-terminal, eliminate x's labelled at root of tree
    \item the resulting BDD is 1) 0: not realizable, 2) not 0: partially realizable
\end{enumerate}

\subsection{Synthesis}
\begin{enumerate}
    \item 

    \item build the graded tree (X closer to root, Y farther) where a leave represents a factor

    \item conjunt with a new leave at a time, then on every internal node eliminate y's that occur for the last time and apply synthesis
\end{enumerate}



==> sections/subsec4.1_old.tex <==
\subsection{Monolithic Approach and Clustering}\label{subsec: monolithic and clustering}

\subsubsection{Linear Projections in Monolithic Scenario}\label{subsec: witness monolithic}
As a stepping stone towards graded-tree-based synthesis, we first explain how witness functions can be constructed in the monolithic case. We review the basic framework in~\cite{CAV16}, where the realizability set $R_{\phi}$ is obtained through iterative quantification from $y_n$ to $y_1$, while witnesses are obtained via iterative substitution of $y_1$ to $y_n$. 

Denote the BDD encoding the original CNF formula $\phi(X,Y)$ to be $B_\phi(X,Y)$. Denote clauses in the formula by $c_j$.
Denote the set of clauses that have occurrences of variables $x$ by $T_x$.

Then a series of intermediate BDDs can be defined on the way of obtaining the realizability sets $R_\phi$:

\begin{align*}\centering
    &B_n(X, y_1, \ldots, y_n) 
    \equiv \llbracket \bigwedge_i c_j \rrbracket;\\
    &B_{n-1}(X, y_1, \ldots, y_{n-1}) 
    \equiv (\exists y_n)B_n 
    \equiv \llbracket \bigwedge_{c_j \not\in T_{y_n}} c_j \rrbracket \land \left( (\exists y_n)\llbracket\bigwedge_{c_j \in T_{y_n}} c_j\rrbracket \right),\\
    &\textit{where the }c_j\textit{'s denote the clauses in } B_n;\\
    %&B_{n-2}(X,Y)=B_{n-2}(X, y_1, \ldots, y_{n-2}) \equiv (\exists y_{n-1})(\exists y_n) B_n \textit{, which is a function of $X, y_1, \ldots, y_{n-2}$;}\\
    &\ldots\\
    &B_{i}(X, y_1, \ldots, y_i) 
    \equiv (\exists y_{i+1})\ldots(\exists y_n)B_n
     \equiv \llbracket \bigwedge_{c_j \not\in T_{y_{i+1}}} c_j \rrbracket \land \left( (\exists y_{i+1})\llbracket\bigwedge_{c_j \in T_{y_{i+1}}} c_j\rrbracket \right),\\
    &\textit{where the }c_j\textit{'s denote the clauses in } B_{i+1};\\
    &\ldots\\
    %&B_2(X,Y)=B_{2}(X, y_1, y_2) \equiv (\exists y_{3})\ldots(\exists y_{n})B_n \textit{, which is a function of $X, y_1, y_2$;}\\
    &B_{1}(X, y_1) 
    \equiv (\exists y_{2})\ldots(\exists y_n)B_n 
    \equiv \llbracket \bigwedge_{c_j \not\in T_{y_2}} c_j \rrbracket \land \left( (\exists y_2)\llbracket\bigwedge_{c_j \in T_{y_2}} c_j \rrbracket\right),\\
    &\textit{where the }c_j\textit{'s denote the clauses in } B_2;\\
    &B_{0}(X) 
    \equiv (\exists y_{1})\ldots(\exists y_n)B_n 
    \equiv \llbracket \bigwedge_{c_j \not\in T_{y_1}} c_j \rrbracket \land \left( (\exists y_1)\llbracket\bigwedge_{c_j \in T_{y_1}} c_j\rrbracket \right),\\
    &\textit{where the }c_j\textit{'s denote the clauses in } B_1.\\
\end{align*}
After each step of existential projections on a particular $y_i$, we conjoin the clauses that have occurrences of the next variable to be projected, and leave the other clauses as they are. As indicated by the $\llbracket \cdot \rrbracket$ notation, we perform projections only on the BDD representing the conjunction of the part of clauses involving the particular variable. We call this feature \emph{only necessary conjoining}. Similarly in synthesis, we never perform conjunction operations when we do not have to.

In general, we have 
$B_{i-1}
\equiv(\exists y_n)\ldots(\exists y_i)B_n
\equiv(\exists y_i)B_{i}$ and
$R_\phi(X)=B_0(X)$ is the realizability set.
We call this the \emph{outside-in} framework for realizability, because larger indexed output variables are quantified before smaller indexed output variables. As a result of our \emph{only necessary conjoining} principles, the given problem has full realizability only when all the factoring clauses after projections are equivalent to $1$.

The corresponding synthesis approach under this framework is an \emph{inside-out} solution for computing the functions for witnesses in~\cite{CAV16}. Here, witnesses are constructed in the reverse direction starting from the smallest indexes output variable. Formally, a witness function $g_1$ for $y_1$ is first computed from $B_1(X,y)$, which is the realizability set on $X \cup \{y_1\}.$
%which encodes a function of $X$ variables and $y_1$. 
% A example for $g_{y_1}$ can be $B_1[y_1 \mapsto B_1[y_1 \mapsto 1]$, whose correctness is proved in \cite{CAV16}. 
Next, to construct the witness $g_2$, the witness $g_1$ is first substituted into $B_2(X,y_1,y_2)$. 
Iteratively, we use the witnesses $g_1,\ldots,g_{i-1}$ to construct the next witness $g_i$.
%Iteratively, each time one former witness is being substituted, and the BDDs for functions are produced in this order. 
This framework of applying quantifications and substitutions in reverse order provides the starting point for our graded-tree-based approach below.

We now describe this framework in detail.
%Fix the witness of an output variable $y$ in a BDD $B$, which encodes some formula over a set of variables that includes $y$, to be $g_{y}=B[y \mapsto B[y \mapsto 1]]$ \cite{CAV16}. 
We now have: 
\begin{align*}
    &g_1 \textit{ is computed from } B'_1=B_1: 
     \\ & \hspace{2cm} g_{1}=B'_1[y \mapsto B_1[y_1 \mapsto 1]];\\
    &g_2 \textit{ computed from } B'_2=B_2[y_1 \mapsto g_1]: 
    \\ & \hspace{2cm}g_{2}=B'_2[y_2 \mapsto B'_2[y_2 \mapsto 1]];\\
    &\ldots\\
    &g_{i} \textit{ is computed from } B'_i=B_i[y_{1} \mapsto g_{1}][y_{2} \mapsto g_{2}]\ldots[y_{i-1}\mapsto g_{i-1}]:
   \\ & \hspace{2cm}g_{i}=B'_i[y_i \mapsto B'_i[y_i \mapsto 1]];\\
    &\ldots\\
    &\textit{and }g_{n} \textit{ is computed from } B'_n=B_n[y_{1} \mapsto g_{1}][y_{2} \mapsto g_{2}]\ldots[y_{n-1} \mapsto g_{n-1}]:
    \\ & \hspace{2cm} g_{n}=B'_n[y_n \mapsto B'_n[y_n \mapsto 1]]
\end{align*}

Note that our \emph{only-necessary-conjoining} framework is consistent throughout the synthesis process. $g_i$ computed from substitutions on $y_i$ does not require additional conjoining of clauses.

\begin{lemma}\label{lemma: monolithic correct}{\rm \cite{CAV16}}
The $g_i$'s above provide a satisfying set of witness functions for corresponding variables $y_i \in Y$ in $R_\phi$.
\end{lemma}
\begin{proof}

We prove by induction. Let $P(i)$ state that $g_1,\ldots,g_i$ consist of a set of satisfying assignments to variables $y_1,\ldots, y_i$ in $B_i$.

Base case: When $i=1$, $g_1$ satisfies $B_1'=B_1$, by Lemma.~\ref{lemma: witness one y}. Hence $P(1)$ is true.

Inductive step: Given $P(i)$ for all $i\geq1$, $g_1,\ldots, g_{i}$ satisfy $B_i$. 
Hence $B_i[y_{1} \mapsto g_{1}][y_{2} \mapsto g_{2}]\ldots[y_{i-1}\mapsto g_{i-1}][y_i \mapsto g_i]=1$.
Then $(\exists y_{i+1})B_{i+1}[y_{1} \mapsto g_{1}][y_{2} \mapsto g_{2}]\ldots[y_{i-1}\mapsto g_{i-1}][y_i \mapsto g_i]=1$.
By Lemma.~\ref{lemma: witness one y}, $g_{i+1}$ is a witness of $y_{i+1}$ in $B'_{i+1}=B_{i+1}[y_{1} \mapsto g_{1}][y_{2} \mapsto g_{2}]\ldots[y_i\mapsto g_i]=1$.
Hence $B_{i+1}[y_{1} \mapsto g_{1}][y_{2} \mapsto g_{2}]\ldots[y_{i-1}\mapsto g_{i-1}][y_i \mapsto g_i][y_{i+1}\mapsto g_{i+1}]=1$.
i.e., $P(i+1)$ is also true.
Thus the inductive step is proved.

Therefore $P(n)$ holds for all positive index $i$ of output variables, and the computed witnesses consist of a satisfying assignment to $y$ variables.\qed
\end{proof}

\subsubsection{Clustering Scenario Synthesis}\label{subsec: cluster monolithic}
Before proceeding to develop our graded-tree-based approach for witness synthesis, we consider another algorithmic component. If the clauses are organized into groups, the framework described above is still applicable. Let $c_1, \ldots, c_k$ denote the clauses of CNF $\phi$. We wish to partition the clauses $c_1, \ldots, c_k$ into $m$ \emph{clusters} $T_1, \ldots, T_m$, where each $T_i$ is a conjunction of some clauses. We associate with the cluster $T_j$ the set $out(T_j)$ of the output variables that do not occur in a cluster $T_{j'}$ with $j'>j$. Equivalently speaking, the set $out(T_j)$ consists of the variables that only occur in clusters $T_1, \ldots, T_j$. Moreover, since each $out(T_j)$ includes as many variables as possible that satisfies this criterion, for all $1 \leq j \leq m$, if a variable $y \in out(T_j)$, then there is some clause where $y$ occurs in the cluster $T_j$, and it is guaranteed that $y\not\in out(T_k)$ for all $k\neq j$.  %\myv{Rewrote{$Out(T_j)$}
\yi{done rewriting this part}

 

In detail:
\begin{align*}
    &out(T_1) \textit{ contains all output variables that occur only in clauses in $T_1$},\\
    &\ldots,\\
   % &out(T_j)   \textit{ contains all output variables  that occur only  in clauses in $T_1, \ldots, T_j$},\\
      &out(T_j) \textit{ contains all output variables  that occur in clauses in $T_j$, but not in clauses in $T_{j+1}, \ldots, T_m$},\\
    &\ldots,\\
    %&out(T_{m-1})   \textit{ contains all variables $y$ which only occurs in clauses in $T_1, \ldots, T_{m-1}$},\\
        &out(T_{m})   \textit{ contains all output variables that occur in clauses in $T_{m}$}.\\
\end{align*}
The intuition behind this definition is that an output variable $y\in out(T_j)$  does not depend on the clauses in $T_{j+1},\ldots,T_m$. Thus, these clauses can be ignored when constructing witnesses for $y$. i.e., the values of clauses in other clusters do not affect the functions constructed for this variable.\yi{revised}
%\myv{Suppose we have clauses with no output variables. Where do we consider them?}

We use the notation $\mathcal{B}_i$ to denote the BDD representing the conjunction of clauses in cluster $T_i$.

We now apply the witness-construction process as in Section.~\ref{subsec: witness monolithic}.  
If  $y_i \in out(T_j)$, \myv{What is $l(T_j)$?}\yi{revised}
then we compute its witness from $\mathcal{B}_j$: 
\myv{Why $B_{1,i}$?}\yi{revised}
$\llbracket \mathcal{B}_{j}(X, Y) \rrbracket= \bigwedge_{c \in T_j} c  $, and the witness is $ g_i = \llbracket \mathcal{B}_{j}(X, Y)[y_i \mapsto \mathcal{B}_{j}(X, Y)[y_i \mapsto 1]] \rrbracket.$



Of course, this encodes an expression containing other output variables $y'$, and we treat $\mathcal{B}_{j}(X, Y)$ as the representation of a monolithic formula and use the procedure described in Section.~\ref{subsec: witness monolithic} to get other witnesses for $y'$. Hence,

\begin{align*}
    &\textit{For } y_i \in out(T_1), \llbracket \mathcal{B}_{1}(X, Y)\rrbracket =  \bigwedge_{c \in T_1} c , \textit{We compute its witness by } 
    \\ & \hspace{1cm} g_i =\llbracket \mathcal{B}_{1}(X, Y)[y_i \mapsto \mathcal{B}_{1}(X, Y)[y_i \mapsto 1]]\forall_{\textit{other }y'}[y' \mapsto g_{\textit{monolithic},y'}] \rrbracket.\\
    %&\textit{For } y_i \in out(T_2), B_{2}(X, Y) = \llbracket \bigwedge_{c \in T_1 \cup T_2} c \rrbracket, \textit{We compute its witness by } 
    %\\ & \hspace{1cm} g_i = B_{2}(X, Y)[y_i \mapsto B_{2}(X, Y)[y_i \mapsto 1]]\forall_{\textit{other }y'}[y' \mapsto g_{\textit{monolithic},y'}].\\
    &\ldots\\
    &\textit{For } y_i \in out(T_k), \llbracket \mathcal{B}_{k}(X, Y) \rrbracket= \bigwedge_{c \in T_1\cup \ldots \cup T_k} c , \textit{We compute its witness by }
    \\ & \hspace{1cm} g_i =\llbracket \mathcal{B}_{k}(X, Y)[y_i \mapsto \mathcal{B}_{k}(X, Y)[y_i \mapsto 1]]\forall_{\textit{other }y'}[y' \mapsto g_{\textit{monolithic},y'}] \rrbracket.\\
    &\ldots\\
    &\textit{For } y_i \in out(T_m), \llbracket \mathcal{B}_{m}(X, Y)\rrbracket =  \bigwedge_{c \in T_1\cup \ldots \cup T_m} c , \textit{We compute its witness by }
    \\ & \hspace{1cm} g_i =\llbracket \mathcal{B}_{m}(X, Y)[y_i \mapsto \mathcal{B}_{m}(X, Y)[y_i \mapsto 1]]\forall_{\textit{other }y'}[y' \mapsto g_{\textit{monolithic},y'}] \rrbracket.
\end{align*}
\begin{lemma}\label{lemma: clustering witness}
In the monolithic case, under clustering of clauses into some arbitrary $T_1, \ldots, T_m$, where $m$ is the number of clusters, the constructed witnesses as above compose of a set of assignments to the output variables in $Y$ that satisfies the original CNF $\phi$, as long as the formula is not unsatisfiable.
\end{lemma}
\begin{proof}
By lemma.~\ref{lemma: monolithic correct}, the witnesses $g_{y'}$for other variables are satisfying, and thus do not modify the truth values of $\llbracket \mathcal{B}_{1}(X, Y)\rrbracket,\ldots,\llbracket\mathcal{B}_{m}(X, Y)\rrbracket$. This proves the last substitution operation in each $g_i$. We only need to show the former part of $g_i$, which can be proved by correctness of self-substitution.
\qed
\end{proof}

Next, we consider the tree-based scenario.

==> sections/subsec4.2_old.tex <==
\subsection{Approach Based on Graded Project-Join Trees}\label{subsec: graded pj trees appraoch}

\subsubsection{Construct Witnesses from Modified Tree}\label{subsec: synthesis alg}
%show the process of visiting all the internal nodes and compute witnesses
%put the algorithms and proofs

\begin{lemma}\label{lemma: substitution}
Let $g_{y_i}$ be a BDD representing a satisfying construction of function for variable $y_i$ in $\pi(m)$. Then in the graded project-join tree $\T$, then for all variables $y$ in $\pi(n)$ where $m$ is an ancestor node of $n$, then $\texttt{BV}_{\texttt{pre}}(n)[y_i \mapsto y(y_i)]=1$.
\end{lemma}
\begin{proof}
The lemma follows from Definition.~\ref{def: BDD valuation} and Definition.~\ref{def: witness construction}.
\qed
\end{proof}


We construct the witnesses for outputs in the reverse direction of realizability, i.e., from the variables labelled by higher level internal nodes down to those on direct parents of the leaves, as in Algorithm.~\ref{alg: synth}. The $\texttt{pre-BV}$ for a node in a tree is computed along with Algorithm.~\ref{alg: generic}. This computation is only not operated in the case of early detection on an empty set of $R(\vec{x})$.

Now that we have the picture of mutual relations among the witness functions, we present the dynamic synthesis algorithm of producing $g_y(\vec{x})$ in Algorithm.~\ref{alg: synth}. As analyzed above, we want to substitute the BDDs representing solutions to those output variables in higher level, i.e. closer to the root, into the BDDs of solution functions for output variables with shallower depth in the tree. This idea is presented in the algorithm by the \texttt{UpperYs} function. Equivalently speaking, if $y'$ is in the set $\pi(n')$ and $y$ is in the set $\pi(n)$, and $n'$ is in the descendants of $n$, then $n \in \texttt{UpperYs}(n')$. The set of upper outputs also direct the for-loop in line 5-8 to substitution phase, where by the analysis in Section.~\ref{subsec: dependencies in witnesses} completes the construction of a $g_{y_i}(\vec{x})$ purely expressed by the input variables.

\begin{algorithm}
\caption{${DPSynth}(\T)$}\label{alg: synth}
     \DontPrintSemicolon
     \SetKwFunction{topYs}{XLeaves}
     \SetKwFunction{preBV}{pre-valuation}
     
     \SetKwFunction{syn}{constructWitness}
     \SetKwFunction{laterYs}{UpperYs}
     \SetKwInOut{Parameter}{Notation}
     
     \Parameter{$D(n)$: set of the descendant nodes of $n$}
     \Parameter{$C(n)$: set of the children nodes of $n$}
     \Parameter{$W(y))$: BDD representing the witness of variable $y$}
    % %\SetKwInOut{Parameter}{Notation}
    % \SetKwInOut{function}{Operation}
    
    
    % (1) say sanity check is done by verifysol
    % (2) 1-witness is correct for 1 y
    % (3) when there are multiple y's
    \Parameter{$\llbracket \alpha \rrbracket$: the BDD representation of boolean expression $\alpha$}
    
    \Parameter{$\topYs(\T)$ as in Algorithm.~\ref{alg: low valuation}}
    
    \KwIn{$\T = (T, r, \gamma, \pi)$: the original $(X,Y)$-graded project-join tree of CNF $\phi$.}
    \KwIn{ BDDs $\texttt{pre-valuation}(m)$ for all $m \in \I_Y$}
    
    \KwOut{a series of BDDs $W(y), \forall y \in Y$ encoding the witnesses functions for output variables}
    
    \If{$\I_Y$ is empty}{
        \Return{ }
    }
    $\texttt{synthNodes} \gets \topYs(\T), \texttt{constructionDone} = 0$\;
    \While{\texttt{constructionDone} == 0}{
        \texttt{constructionDone} = 1\;
        \For{$n \in \texttt{synthNodes}$}{
            $\texttt{newsynthNodes} = \{\}$\;
            $\texttt{constructionDone} \gets 1$\;
            \For{$n' \in C(n)$}{
                add $n'$ to \texttt{newsynthNodes}\;
                \texttt{constructionDone} = 0\;
            }
            $\texttt{Y(n)} \gets $the set of Y variables labelled on $n$\;
            \If {$\texttt{Y(n)}$ is empty} {
                continue\;
            } \Else {
                \tcp{compute BDD of witnesses for variables labelled on this node}
                \For{$y \in \texttt{Y(n)}$} {
                    \tcp{using the algorithm presented in Section.~\ref{subsec: monolithic and clustering}}
                    $W(y) \gets Solve(y, n, \T)$ 
                    
                }
                
            }
        }
        $\texttt{synthNodes} \gets \texttt{newsynthNodes}$\;
    }
    
    \For{all synthesized $y $}{
        
        %$\laterYs(y) = \{y' \in Y \mid \pi^{-1}(y') \in D(\pi^{-1}(y)) \}$\;\tcp{$y'$ is labelled on descendants of the node labelling $y$}
        
        \For{all $y'$ that are synthesized later than $y$}{
            \tcp{substitute $y'$ by its witness in the BDD representing the witness of $y$}
            $W(y) \gets W(y)[y' \mapsto W(y')]$\;
        }
    }
    check number and correctness of witnesses using $\texttt{verifySol}$\tcp{in CUDD functionality\cite{CUDD_cudd}}
    \Return{$W(y), \forall y \in Y$}

\end{algorithm}

\paragraph{Selection of Witnesses} The implementation of function \texttt{constructWitness} in line 3 of Algorithm.~\ref{alg: solve} replies on selection of witness functions. In this work for simplicity of comparison we select the 1-witness $f(\vec{x}, f(\vec{x},1))$ in \cite{CAV16} for single dimensional output, and for multidimensional outputs we thereby compute the witnesses by substitutions under this framework. 



Furthermore, we elaborate the function \texttt{solve} in line 4 in the separated Algorithm.~\ref{alg: solve}, because in order to traverse the internal nodes and solve for output variables, the ordering of visiting also makes an impact. Algorithm.~\ref{alg: synth} applies $\texttt{solve}(\T, n)$ from $\texttt{XLeaves}(\T)$ only, which is consisted of the internal nodes in $Y$ partition that are in the highest layer. This leads to the top-down traversal in Algorithm.~\ref{alg: solve} in the while-loop from lines 5 to line 10, where descendants are always added, and therefore the witnesses for variables labelled on $\pi$ functions of those descendant nodes are to be synthesized later, independent of the choice of witness functions. This guarantees that all nodes are visited once, and it is consistent with our original expectation of the synthesis dependencies within the graded tree structure.

The following theorems prove the correctness of witnesses constructed. First, we show in Theorem.~\ref{thm: alg solve} that Algorithm.~\ref{alg: solve} guarantees the production of a function for each output variables. 

\begin{theorem}\label{thm: alg solve}
Given node $n$ in the set of uppermost $Y$ internal nodes of a graded project-join tree $\T$, then for all variables $y_i$ in $\pi(m)$ where $m$ is a descendant of $n$, a witness function $g_{y_i}(\vec{x})$ is computed by Alg.~\ref{alg: solve} by \texttt{constructWitness}.
\end{theorem}
\begin{proof}
Let $y_i$ be an arbitrary variable labelled on $m$ in descendants of $n$. Under the given conditions, it is clear that before node $m$ is visited in line 6, the set $Q$ is never empty. Since the first iteration all children of $n$ are included but in all later iterations only the strict children reside in $Q$ as line 10 operates. Hence first we know that there exists an iteration of the for-loop in line 6-9 where $n'=m$. 

Next, $b$ is assigned to the BDD of $\texttt{BV}_\texttt{pre}(m)$, and by the supposition $y_i$ must be in $\pi(m)$ and hence a function for witnesses is constructed in line 9. 
\qed
\end{proof}
 Next we show the correctness of witnesses constructed.
 
 \begin{theorem}\label{thm: alg synth}
Alg.~\ref{alg: synth} returns a set of BDDs encoding the witness functions for output variables that satisfy the given CNF, given that a correct $\texttt{constructWitness}$ function is selected in Alg.~\ref{alg: solve}.
\end{theorem}
\begin{proof}
For simplicity and consistency of comparison, we select the 1-witness $f(\vec{x}, f(\vec{x},1))$ in \cite{CAV16} for one dimensional $y$ variables, as explained above. Substitutions are performed on the variables labelled on the same node only, but there are other output variables labelled on other internal nodes in the functions generated.

Here we want to show the new way of constructing witnesses that the graded project-join tree structure provides also generates a set of satisfying functions. 

Let $y_i \in \texttt{XLeaves}$ be arbitrary in line 3. First we know under the assumption that the witnesses \texttt{solve} returns only guarantees the pre-valuations of the subtree under the node $n= \pi^{-1}(y_i)$ which $y_i$ is labelled on. Then the computed witness function $g_{y_i}$ satisfies $\texttt{BV}_\texttt{pre}(\pi^{-1}(y_i))[y_i \mapsto g_{y_i}]=1$. Moreover, for this arbitrary $y_i$, the pre-valuation of its node only contains variables labelled on the ancestors of this node. During the inter-node substitutions performed in line 8, all the output variables $y$ are either in $\texttt{UpperYs}(y)$ or have already been substituted in $\texttt{solve}(\T, n)$. Hence the expression encoded by the constructed BDD $g_{y_i}$ is purely dependent on $X$ variables. 

% \todo{Yi: not so sure if this proof is sufficient}
Next, we know $\texttt{BV}_\texttt{pre}(n)\forall_{{y_i} \in \pi(n)}[y_i \mapsto g_{y_i}]=1$, and $\texttt{BV}_\texttt{pre}(n)$ be Definition.~\ref{def: BDD valuation} is equivalent to the conjunction of all leaves under $n$ where all output variables labelled on descendants of $n$ are quantified. 

We proof the correctness by induction. Suppose that the witnesses under $n$ are correct. In the base case, $n$ is a leave, so the correctness is ensured by the selected witness. For example, our implementation uses the 1-witness in \cite{CAV16}. Since the leave representing the only clause that has occurrences of this variable, the witness function satisfies the entire formula no matter what the other variables are, as long as the CNF is realizable, as checked in Alg.~\ref{alg: low valuation} and~\ref{alg: high valuation}.

For induction step, There are two cases for the other output variables $y'$ that occur in the pre-valuation formula. 
\emph{Case 1}: $y'$ is existential quantified. i.e., $y'$ is labelled on a strict descendant of $n$. Then in $\texttt{BV}_\texttt{pre}(n)$, $y'$ has been eliminated, and the witness for it is computed and by inductive hypothesis is correct.
\emph{Case 2}: $y' \in \pi(n)$. Then the pre-valuation is a function of $y'$ and other labelled variables on $n$. The constructed witness satisfies $\texttt{BV}_\texttt{pre}(n)$, and additionally $y'$ is one of the $y' \in \pi(n)$ in $\texttt{BV}_\texttt{pre}(n)\forall_{{y_i} \in \pi(n)}[y' \mapsto g_{y'}]=1$. Then the constructed witnesses of $y'$, along with previous witnesses labelled on descendants of $n$, compose of a partial set of assignments to output variables that satisfy the conjunctions of clauses represented by leaves under this current node. This partial set does not guarantee other clauses to be satisfied, but as long as there is some satisfying set of assignments to the entire CNF, this set must be part of one of the satisfying set. i.e., the construction of the witness $g_{y'}$ is correct.

Now we know that the witnesses under $y_i$ are correct. Since inner-node variables and inter-node variables are correct by analysis above, the generated $g_{y_i}$ satisfies the conjunction of all clauses under $n$ and therefore is a correct witness iff $R(x)\neq\emptyset$. Thus we have the correctness of arbitrary $g_{y_i}$.
\qed
\end{proof}


\subsubsection{Graded-Tree Based Synthesis}\label{subsec: witness in tree}
% graded-tree path eliminate

Before we analyze as in previous subsections, let us consider the unique features of the graded-tree perspective to the synthesis problem.

From the perspective of a graded tree, the dependencies from the functions for witnesses are therefore transferred to more the nodes in the tree than those in the BDDs. As analyzed in previous sections, the projections on $Y$-partition variables can be completely linear if the graded-tree is a perfect left-leaning tree. i.e., each level in the graded tree only has at most one $Y$ internal nodes, and the leaves under $Y$ internal nodes are always on the right-side child except for the deepest level. We say our tree-based realizability checking is \emph{bottom-up}, as in Algorithm.~\ref{alg: low valuation}, as its actual steps start from computing the \texttt{pre-} and \texttt{post-valuations} from the leaves to the top. Now we can have the approach to witness construction which dynamically utilizes the tree structure. We call this approach \emph{top-down} as it visits the $Y$ internal nodes from \texttt{XLeaves} to the leaves. 


We put with specific notations to explain the idea formally.
Let $n$ be an $Y$ internal node in the \texttt{XLeaves} of the graded tree $\T$ for the given CNF. i.e., the parent of $n$ is not in the $Y$ partition of internal nodes. We denote the set of output variables labelled on $n$ to be $\pi(n)$, the set of children of $n$ to be $C(n)$, the descendants of $n$ to be $D(n)$.

\begin{itemize}
    \item[1.] Compute its \texttt{pre-valuation}, which is a BDD representing the conjunction of conditions that evaluates all clauses in its descendants to be true. As previously defined,
    
    $$\texttt{BV}_{\texttt{pre}}(n)=
        \begin{cases}
			\llbracket \gamma(n) \rrbracket & \text{if $n$ is a leaf node,}\\
               \bigwedge_{n' \in C(n)}  \texttt{BV}_{\texttt{post}}(n')      & \text{if $n$ is an internal node.}
		 \end{cases}.$$
    \item[2.] Then we apply the synthesis formula on this BDD to get witnesses for variables labelled on this node.
    
    In other words, for a variable $y_i$ labelled on node $n$, we first compute the witnesses of other variables labelled on $n$ by the algorithm in Section.~\ref{subsec: witness monolithic}, treating $\texttt{BV}_{\texttt{pre}}(n)$ as a monolithic function.
    
    Then we get the witnesses of $y_i$ by 
    
    $g_i =\texttt{BV}_{\texttt{pre}}(n)[y_i \mapsto \texttt{BV}_{\texttt{pre}}(n)[y_i \mapsto 1]]\forall_{\textit{other }y' \in \pi(n)}[y' \mapsto g_{{monolithic}, y'}] $, where the witnesses of other $y' \in \pi(n)$ are substituted.
    
    \item[3.] Next go one level down, and repeat the procedure on its children nodes, iteratively, until we have computed the witnesses $g_{y''}$ for variables $y'' \in \pi(n'), n' \in D(n)$ labelled on the descendants of $n$.
    \item[4.] Substitute the witnesses for variables labelled on upper levels into the functions for variables on lower levels.
    
    i.e., $g_i = g_i\forall_{\exists n' \in D(n), y'' \in \pi(n')}y''[y'' \mapsto g_{y''}].$
\end{itemize}

\begin{lemma}\label{lemma: tree-based witness}
For a graded project-join tree $\T$ for CNF $\phi$, the above procedure generates a set of satisfying witness functions for $y_i, \forall i.$ 
\end{lemma}
\begin{proof}
Let $y_i$ be an arbitrary output variable in $\phi$. Its witness constructed is $$g_i = g_\textit{internode}\forall_{\exists n' \in D(n) \textit{s.t.} y'' \in \pi(n')}y''[y'' \mapsto g_{y''}],$$ where \begin{align*}
    &g_\textit{internode}=g_w\forall_{y' \in \pi(n), y' \neq y}[y' \mapsto g_{monolithic, y'}],\\
  \textit{ and } &g_w=\texttt{BV}_{\texttt{pre}}(n)[y_i \mapsto \texttt{BV}_{\texttt{pre}}(n)[y_i \mapsto 1]].
\end{align*}
First, the correctness of $g_w$ follows from lemma~\ref{lemma: witness one y}. Next, $g_\textit{internode}$ is correct by lemma~\ref{lemma: monolithic correct}. Finally, we need to show the mappings $[y'' \mapsto g_{y''}]$, for all $y''$ labelled on some descendants of $n$, does not affect the truth value of $g_i$. This can be proved by induction on the hypothesis that $g_i$ is correct on all level of nodes below $n$ in the tree, and the base case can be the leave level nodes. Hence we have proved the $g_i$'s constructed from the steps above gives a set of witness functions for output variables.
\qed
\end{proof}

%section 4.4 and 4.5:
%simplify explanations in 4.4
%modify the proofs in 4.5 by referring to lemmas in 4.1-4.3
%revise the algs in 4.5


\subsubsection{Dependencies among Witnesses}\label{subsec: dependencies in witnesses}
% the role of preVal in synthesis
% dependencies of witnesses in higher nodes on witnesses in lower nodes, 
The transformation of the CNF formula into a graded project-join tree restructures the conjunction of constraints into clusters of clauses. Utilizing this feature, output variables are aligned from upper level to lower level internal nodes in the graded tree, such that those which are labelled on descendant internal nodes have common occurrences with those that are labelled on the ancestor internal nodes, but the converse is not true.

This brings convenience in constructing BDDs representing the witness functions, as the problem of synthesis in boolean context aims to generate a set of functions for output variables from given input variable values.






First, we want to understand the mutual or unidirectional dependencies among witness functions. In producing the witness functions of output variables from the internal nodes labelling them, boolean witnesses functions can be generated as equivalent representations. A witness function generated, in ideal case, is necessarily never dependent upon other witness functions that depend on itself. Computing the witnesses in the order of the single direction of dependencies, the solution matrix of output variables $\vec{y}$ is generated.

\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=0.15]
\tikzstyle{every node}+=[inner sep=0pt]
\draw [black] (36,-8.5) circle (3);
\draw (36,-8.5) node {$10$};
\node[below] at (44,-8.5) {$e: x_1,x_2$};
\draw [black] (27.6,-18.6) circle (3);
\draw (27.6,-18.6) node {$8$};
\node[below] at (33.6,-18.6) {$e: x_3$};
\draw [black] (43,-19.1) circle (3);
\draw (43,-19.1) node {$9$};
\node[below] at (49,-19.1) {$e: y_6$};
\draw [black] (21.2,-28.1) circle (3);
\draw (21.2,-28.1) node {$7$};
\node[below] at (27.2,-28.1) {$e: y_5$};
\draw [black] (61.2,-29.2) circle (3);
\draw (61.2,-29.2) node {$3$};
\node[below,align=left] at (61.2,-33.2) {$(\neg x_1 \lor x_2 \lor y_6)$};
\draw [black] (34.1,-43.9) circle (3);
\draw (34.1,-43.9) node {$5$};
\node[below,align=left] at (34.1,-47.9) {$(x_1 \lor \neg x_2 \lor x_3 \lor y_5)$};
\draw [black] (47.3,-41.3) circle (3);
\draw (47.3,-41.3) node {$2$};
\node[below,align=left] at (47.3,-45.3) {$(\neg x_3 \lor x_2 \lor \neg y_5)$};
\draw [black] (20.4,-51.5) circle (3);
\draw (20.4,-51.5) node {$4$};
\node[below,align=left] at (21,-55.5) {$(\neg x_3 \lor x_1 \lor \neg y_4)$};
\draw [black] (7.6,-51.5) circle (3);
\draw (7.6,-51.5) node {$1$};
\node[below,align=left] at (5,-55.5) {$(x_1 \lor y_4 \lor \neg y_5)$};
\draw [black] (13.5,-36.3) circle (3);
\draw (13.5,-36.3) node {$6$};
\node[below] at (19.5,-36.3) {$e: y_4$};
\draw [black] (37.65,-11) -- (41.35,-16.6);
\fill [black] (41.35,-16.6) -- (41.32,-15.65) -- (40.49,-16.2);
\draw [black] (34.08,-10.81) -- (29.52,-16.29);
\fill [black] (29.52,-16.29) -- (30.41,-16) -- (29.65,-15.36);
\draw [black] (25.7,-21.1) -- (22.82,-25.58);
\fill [black] (22.82,-25.58) -- (23.68,-25.17) -- (22.83,-24.63);
\draw [black] (45.62,-20.56) -- (58.58,-27.74);
\fill [black] (58.58,-27.74) -- (58.12,-26.92) -- (57.63,-27.79);
\draw [black] (23.1,-30.42) -- (32.2,-41.58);
\fill [black] (32.2,-41.58) -- (32.08,-40.64) -- (31.31,-41.27);
\draw [black] (23.88,-29.45) -- (44.62,-39.95);
\fill [black] (44.62,-39.95) -- (44.13,-39.14) -- (43.68,-40.03);
\draw [black] (12.6,-39.3) -- (10.32,-48.59);
\fill [black] (10.32,-48.59) -- (10.99,-47.93) -- (10.02,-47.69);
\draw [black] (14.74,-39.03) -- (19.16,-48.77);
\fill [black] (19.16,-48.77) -- (19.28,-47.83) -- (18.37,-48.25);
\draw [black] (18.8,-30) -- (15.43,-34);
\fill [black] (15.43,-34) -- (16.33,-33.71) -- (15.56,-33.07);
\end{tikzpicture}
\caption{Graded Project-join Tree For CNF Example}
\label{fig: tree}
\end{center}
\end{figure}

Solving for a particular output variable at a node, the conjunction of all clauses having occurrences of the variable consist of a boolean formula that we use to solve for the witness function. Since other clauses are not affected by the value of this particular output variable to be solved, the witness function generated from these clauses also satisfies the overall CNF. Moreover, applying existential quantification on other variables to this conjunction also do not have influence on the condition to the witness function. The definition of pre-valuations in Section.~\ref{sec: realizability(new)} exactly takes this role. 


Now we look at how a construction of $g_y(\vec{x})$ for a particular $y$ rely on witness functions of other output variables. As an instance, Figure.~\ref{fig: tree} illustrates a graded project-join tree of CNF $(x_1 \lor y_4 \lor \neg y_5) \land (\neg x_3 \lor x_2 \lor \neg y_5) \land (\neg x_1 \lor x_2 \lor y_6) \land (\neg x_3 \lor x_1 \lor \neg y_4) \land (x_1 \lor \neg x_2 \lor x_3 \lor y_5)$. In this example, a satisfying construction of witness \cite{CAV16} for $y_5$ is $g_5(\vec{x})=\texttt{BV}_{\texttt{pre}}(n_7)[y_5 \mapsto (\texttt{BV}_{\texttt{pre}}(n_7)[y_5 \mapsto 1])]$. Similarly, a witness for $y_4$ in the same set of satisfying truth assignments that assigns the overall CNF to 1 is $g_4(\vec{x})=\texttt{BV}_{\texttt{pre}}(n_6)[y_4 \mapsto (\texttt{BV}_{\texttt{pre}}(n_6)[y_4 \mapsto 1])]$. It is obvious in this tree that the value of $g_4(\vec{x})$ is dependent upon $g_5(\vec{x})$, on the grounds that by definitions $\texttt{BV}_{\texttt{pre}}(n_7)=(\exists y_4)(l_1 \land l_4) \land l_5 \land l_2$ and $\texttt{BV}_{\texttt{pre}}(n_6)=(l_1 \land l_4).$ Thus the witnesses of variables on lower level nodes is consequently computed by substituting the witnesses of variables labelled by upper level nodes. Thanks to the tree structure, the dependence is unidirectional. i.e., for all internal nodes $n_p$ and $n_q$, for all nonnegative integer $d_p < d_q$, for all output variables $y_p$ and $y_q$, if $n_p$ has depth $d_p$ and $n_q$ has depth $d_q$ in the same graded project-join tree, $y_p \in \pi(n_p)$ and $y_q \in \pi(n_q)$, then  $g_{y_q}(\vec{x})$ is dependent on $g_{y_p}(\vec{x})$.

Therefore we eliminate the outputs variables, as in \cite{CAV16}, one at a time. Under the graded-tree encoding of the formula in our specific case, we perform the quantifications from the outermost to the innermost among output variables in $Y$. i.e., to solve for a variables $y_i$, we replace an output variable $y_{i+1}$ in a BDD of the constraints for a witness that evaluates to true, by its witness $g_{y_{i+1}}$, where $y_{i+1}$ is synthesized ahead of $y_i$ as it is labelled in some ancestor nodes of the latter, by substitution operations. Each time we operate this procedure in order to produce the witness BDDs that are purely dependent on the inputs variables.


















  
